Inferring Versatile Behavior from Demonstrations by Matching Geometric Descriptors

Humans intuitively solve tasks in versatile ways, varying their behavior in terms of trajectory-based planning and for individual steps. Thus, they can easily generalize and adapt to new and changing environments. Current Imitation Learning algorithms often only consider unimodal expert demonstrations and act in a state-action-based setting, making it difficult for them to imitate human behavior in case of versatile demonstrations. Instead, we combine a mixture of movement primitives with a distribution matching objective to learn versatile behaviors that match the expert's behavior and versatility. To facilitate generalization to novel task configurations, we do not directly match the agent's and expert's trajectory distributions but rather work with concise geometric descriptors which generalize well to unseen task configurations. We empirically validate our method on various robot tasks using versatile human demonstrations and compare to imitation learning algorithms in a state-action setting as well as a trajectory-based setting. We find that the geometric descriptors greatly help in generalizing to new task configurations and that combining them with our distribution-matching objective is crucial for representing and reproducing versatile behavior.

==> figures/results/box/component_trendline_target_distance_penalty_mTrain_c0.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Number of Training Contexts},
xmajorgrids,
xmin=1.95, xmax=25.05,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Mean Distance to Target [m]},
ymajorgrids,
ymin=0.00457170459472248, ymax=0.122342733726559,
ymode=log,
ytick style={color=black},
ytick={0.0001,0.001,0.01,0.1,1,10},
yticklabels={
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\)
}
]
\path [draw=steelblue31119180, fill=steelblue31119180, opacity=0.2]
(axis cs:3,0.00695231870604929)
--(axis cs:3,0.00553100915894002)
--(axis cs:6,0.00578119129200158)
--(axis cs:12,0.00554980028327674)
--(axis cs:18,0.00530841080899071)
--(axis cs:24,0.00536298167176322)
--(axis cs:24,0.00617576690970842)
--(axis cs:24,0.00617576690970842)
--(axis cs:18,0.00595366302797789)
--(axis cs:12,0.00672802234592616)
--(axis cs:6,0.00701120217327338)
--(axis cs:3,0.00695231870604929)
--cycle;

\path [draw=darkorange25512714, fill=darkorange25512714, opacity=0.2]
(axis cs:3,0.0503246222957859)
--(axis cs:3,0.0151533099101683)
--(axis cs:6,0.0348604155600913)
--(axis cs:12,0.0330064221176415)
--(axis cs:18,0.0304092003981429)
--(axis cs:24,0.0375944273205086)
--(axis cs:24,0.0503741638803796)
--(axis cs:24,0.0503741638803796)
--(axis cs:18,0.0450087776596635)
--(axis cs:12,0.0424830262005074)
--(axis cs:6,0.0513426569777397)
--(axis cs:3,0.0503246222957859)
--cycle;

\path [draw=crimson2143940, fill=crimson2143940, opacity=0.2]
(axis cs:3,0.0491506495814192)
--(axis cs:3,0.0234268769753268)
--(axis cs:6,0.032486866698731)
--(axis cs:12,0.0386242461117925)
--(axis cs:18,0.0390855344665381)
--(axis cs:24,0.0414000901108271)
--(axis cs:24,0.0498779436208563)
--(axis cs:24,0.0498779436208563)
--(axis cs:18,0.0458355129452846)
--(axis cs:12,0.0512477484705574)
--(axis cs:6,0.0504601314633506)
--(axis cs:3,0.0491506495814192)
--cycle;

\path [draw=mediumpurple148103189, fill=mediumpurple148103189, opacity=0.2]
(axis cs:3,0.0673924539153605)
--(axis cs:3,0.0246992121461312)
--(axis cs:6,0.0372412372656033)
--(axis cs:12,0.0478221040714644)
--(axis cs:18,0.0482702305430252)
--(axis cs:24,0.0540240064509501)
--(axis cs:24,0.105363894776441)
--(axis cs:24,0.105363894776441)
--(axis cs:18,0.0869800313598908)
--(axis cs:12,0.0818105746213527)
--(axis cs:6,0.0840775545255235)
--(axis cs:3,0.0673924539153605)
--cycle;

\addplot [semithick, black, dashed, forget plot]
table {%
3 0.00758827236363636
24 0.00758827236363636
};
\addplot [semithick, black, dotted, forget plot]
table {%
3 0.0712566969090909
24 0.0712566969090909
};
\addplot [semithick, steelblue31119180, forget plot]
table {%
3 0.00624166393249466
6 0.00639619673263748
12 0.00613891131460145
18 0.0056310369184843
24 0.00576937429073582
};
\addplot [semithick, darkorange25512714, forget plot]
table {%
3 0.0327389661029771
6 0.0431015362689155
12 0.0377447241590744
18 0.0377089890289032
24 0.0439842956004441
};
\addplot [semithick, crimson2143940, forget plot]
table {%
3 0.036288763278373
6 0.0414734990810408
12 0.044935997291175
18 0.0424605237059114
24 0.0456390168658417
};
\addplot [semithick, mediumpurple148103189, forget plot]
table {%
3 0.0460458330307459
6 0.0606593958955634
12 0.0648163393464086
18 0.067625130951458
24 0.0796939506136955
};
\end{axis}

\end{tikzpicture}


==> tikz/dummy.tex <==
% this needs to be hear the appease the tikz gods.
